Beyond Coarse-Grained Matching in Video-Text Retrieval

Video-text retrieval has seen significant advancements, yet the ability of models to discern subtle differences in captions still requires verification. In this paper, we introduce a new approach for fine-grained evaluation. Our approach can be applied to existing datasets by automatically generating hard negative test captions with subtle single-word variations across nouns, verbs, adjectives, adverbs, and prepositions. We perform comprehensive experiments using four state-of-the-art models across two standard benchmarks (MSR-VTT and VATEX) and two specially curated datasets enriched with detailed descriptions (VLN-UVO and VLN-OOPS), resulting in a number of novel insights: 1) our analyses show that the current evaluation benchmarks fall short in detecting a model's ability to perceive subtle single-word differences, 2) our fine-grained evaluation highlights the difficulty models face in distinguishing such subtle variations. To enhance fine-grained understanding, we propose a new baseline that can be easily combined with current methods. Experiments on our fine-grained evaluations demonstrate that this approach enhances a model's ability to understand fine-grained differences.

==> ablation1.tex <==
\begin{table}[]
\caption{\textbf{Performance on UVO}. }
\label{tab:sec7_uvo}
\centering
\scalebox{0.75}{
\begin{tabular}{llrllllllllllll}
\toprule
\multirow{4}{*}{Method} & \multirow{4}{*}{Training-strategy} & \multicolumn{7}{c}{Coarse-grained Evaluation} &  & \multicolumn{5}{c}{Fine-grained Evaluation} \\
\cline{3-9} \cline{11-15}
 &  & \multicolumn{3}{c}{\multirow{1}{*}{T2V}} &  & \multicolumn{3}{c}{\multirow{1}{*}{V2T}} &  & \multirow{3}{*}{noun} & \multirow{3}{*}{adj} & \multirow{3}{*}{verb} & \multirow{3}{*}{adv} & \multirow{3}{*}{prep} \\
\cline{3-5} \cline{7-9}
 &  & \multirow{2}{*}{R@1} & \multirow{2}{*}{R@5} & \multirow{2}{*}{R@10} &  & \multirow{2}{*}{R@1} & \multirow{2}{*}{R@5} & \multirow{2}{*}{R@10} &  &  &  &  &  &  &  &  \\ \hline
\multirow{5}{*}{Frozen} & Coarse & 19.0 & 41.9 & 55.0 &  & 19.2 & 42.0 & 55.1 &  & 6.61 & 7.22 & 9.06 & 9.08 & 8.88 \\
 & Word-neg & 18.6 & 40.3 & 52.8 &  & 17.4 & 40.4 & 53.2 &  & 2.09 & 2.73 & 1.38 & 4.53 & 2.47 \\
 & Phrase-neg &  &  &  &  &  &  &  &  &  &  &  &  &  \\
 & Word-vpt &  &  &  &  &  &  &  &  &  &  &  &  &  \\
 & Phrase-vpt &  &  &  &  &  &  &  &  &  &  &  &  &  \\ \hline
\multirow{5}{*}{TS2-Net} & Coarse & 20.9 & 43.0 & 53.8 &  & 30.9 & 59.5 & 71.9 &  & 6.00 & 6.00 & 7.06 & 10.18 & 8.64 \\
 & Word-neg & 21.3 & 42.4 & 53.7 &  & 24.9 & 52.5 & 64.8 &  & 1.46 & 1.09 & 5.77 & 2.40 \\
 & Phrase-neg & 21.2 & 42.6 & 53.9 &  & 24.3 & 51.4 & 64.1 &  & 1.45 & 1.09 & 5.64 & 2.44 \\
 & Word-vpt &  &  &  &  &  &  &  &  &  &  &  &  &  \\
 & Phrase-vpt &  &  &  &  &  &  &  &  &  &  &  &  &  \\ \hline
\multirow{5}{*}{X-CLIP} & Coarse & 22.9 & 44.6 & 55.6 &  & 33.5 & 62.5 & 74.2 &  & 5.99 & 6.08 & 7.16 & 10.60 & 8.51 \\
 & Word-neg & 21.9 & 43.9 & 54.2 &  & 24.9 & 52.6 & 64.9 &  & 1.30 & 1.41 & 1.09 & 5.49 & 2.28 \\
 & Phrase-neg & 21.8 & 43.7 & 55.0 &  & 29.8 & 57.8 & 69.8 &  & 1.51 & 2.28 & 1.24 & 6.84 & 3.28 \\
 & Word-vpt & 21.5 & 42.4 & 53.9 &  & 30.1 & 58.4 & 70.7 &  & 1.38 & 1.48 & 1.12 & 5.15 & 2.33 \\
 & Phrase-vpt &  &  &  &  &  &  &  &  &  &  &  &  &  \\ \hline
\multirow{5}{*}{UCoFiA} & Coarse & 21.4 & 43.1 & 54.7 &  & 30.7 & 59.6 & 72.8 &  & 5.69 & 6.21 & 7.16 & 10.31 & 8.43 \\
 & Word-neg & 21.1 & 42.2 & 53.7 &  & 22.2 & 48.4 & 61.1 &  & 1.30 & 1.42 & 1.07 & 5.50 & 2.28 \\
 & Phrase-neg & 21.0 & 42.3 & 54.0 &  & 27.3 & 54.8 & 67.8 &  & 1.46 & 2.22 & 1.20 & 3.76 & 3.12  \\
 & Word-vpt & 21.4 & 43.8 & 54.8 &  & 29.0 & 58.1 & 70.2 &  & 1.42 & 1.52 & 1.21 & 5.65 & 2.31  \\
 & Phrase-vpt &  &  &  &  &  &  &  &  &  &  &  &  &  \\ \bottomrule
\end{tabular}}
\end{table}

==> discard.tex <==
Early methods used pre-trained visual and text feature extractor to obtain offline video and text features \cite{bmvc2018vsepp,wray2019JPoSE,chen2020hgr,LiXirong2019W2VVPP,Dong2021DE_hybrid,liu2019ce,dzabraev2021mdmmt,dzabraev2021mdmmt}. 

VSE++ \cite{bmvc2018vsepp} is inspired by hard negative mining, the use of hard negatives in structured prediction, and ranking loss functions. It calculates the difference in similarity between each sample's positive pair and its hardest negative, and uses a hyperparameter to control the margin between positive and negative examples, proposing an improved triplet ranking loss. Most of these methods are based on this loss to optimize the model. Some works also focus on cross-modal fine-grained retrieval between text and video.

JPoSE \cite{wray2019JPoSE} considers entities with different actions (verbs or verb phrases) performed on the same object (noun) as relevant entities. This allows for the construction of both cross-modal and within-modal losses. Specifically, when calculating within-modal losses, relevant entities (text) are treated as positive examples, and the corresponding videos for the same text are also treated as positive examples, while others are treated as negative examples.

HGR \cite{chen2020hgr} represents actions with verbs and entities with noun phrases. It employs different levels of text to guide video encoding into corresponding hierarchical embeddings to distinguish various aspects in videos.

Nowadays, benefits from the success of large vision/vision-language pre-training models \cite{vit2021,2021clip_icml}, a series of recent methods highlight the advantages of end-to-end training \cite{bain2021frozen,li2022alpro,luo2022clip4clip,ts2net,xclip}. 

==> fig-cap.tex <==
\begin{wrapfigure}{r}{0.4\textwidth}
    \centering
   \vspace{-2em}
    % \hfill % 添加空间或者可以使用 \quad 
    %\hspace{3mm} 
    \begin{subfigure}[b]{\linewidth}
        \includegraphics[width=\textwidth]{fig1_captions.pdf}
        \caption{\textbf{VATEX}}
        \label{fig:sub2}
    \end{subfigure}
    \vspace{-1.8em}
    \caption{\textbf{Analysis of Sentence Similarity.} Few captions differ by only one part-of-speech. Nouns are the most common cause of fine-grained differences in current benchmarks.}
    \vspace{-4em}
     \label{fig:captions}
\end{wrapfigure}

==> fig-coarse-sumR_bar-baseline.tex <==
\begin{figure}
    \centering
   
    \begin{subfigure}[b]{0.47\textwidth}
        \includegraphics[width=\textwidth]{t2v_coarse_sumR_bar_baseline.pdf}
        \caption{Text-to-Video}
        \label{fig:sub1-t2v}
    \end{subfigure}
    % \hfill % 添加空间或者可以使用 \quad 
    \hspace{4mm} 
    \begin{subfigure}[b]{0.47\textwidth}
        \includegraphics[width=\textwidth]{v2t_coarse_sumR_bar_baseline.pdf}
        \caption{Video-to-Text}
        \label{fig:sub2-v2t}
    \end{subfigure}
 

    \caption{\textbf{Coarse-grained evaluation on the Re-purposed Datasets.}\textbf{Metric: \textit{Sum of Rank@1,5,10 ($\uparrow$})}}
     \label{fig:fine_coarse_sumR_bar_baseline}
\end{figure}

==> fig-fine_eval_bar-baseline.tex <==
\begin{figure}
    \centering
   
    \begin{subfigure}[b]{0.47\textwidth}
        \includegraphics[width=\textwidth]{eccv2024/MSR-VTT_posrank_barchart.pdf}
        \caption{MSR-VTT}
        \label{fig:sub1}
    \end{subfigure}
    % \hfill % 添加空间或者可以使用 \quad 
    \hspace{4mm} 
    \begin{subfigure}[b]{0.47\textwidth}
        \includegraphics[width=\textwidth]{eccv2024/VATEX_posrank_barchart.pdf}
        \caption{VATEX}
        \label{fig:sub2}
    \end{subfigure}
    % \hfill % 添加空间
     \hspace{4mm} 
    \begin{subfigure}[b]{0.47\textwidth}
        \includegraphics[width=\textwidth]{eccv2024/UVO_posrank_barchart.pdf}
        \caption{VLN-UVO}
        \label{fig:sub3}
    \end{subfigure}
    % \hfill % 添加空间
       \hspace{4mm} 
    \begin{subfigure}[b]{0.47\textwidth}
        \includegraphics[width=\textwidth]{eccv2024/OOPS_posrank_barchart.pdf}
        \caption{VLN-OOPS}
        \label{fig:sub4}
    \end{subfigure}

    \caption{\textbf{Fine-grained evaluation on the Re-purposed Datasets.} The four models were retrained, with all hyper-parameters consistent with the original settings except for the batch size, which was set to $256$ in the experiments. \textbf{Metric: \textit{PoSRank ($\downarrow$})}}
     \label{fig:fine_eval_bar_baseline}
\end{figure}

==> fig-fine_eval_radar.tex <==
\begin{figure}

    \centering
    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{eccv2024/msrvtt_radar.jpg}
        \caption{MSR-VTT}
        \label{fig:sub1}
    \end{subfigure}
\hfill
    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{eccv2024/vatex_radar.jpg}
        \caption{VATEX}
        \label{fig:sub2}
    \end{subfigure}
  \hfill
    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{eccv2024/uvo_radar.jpg}
        \caption{VLN-UVO}
        \label{fig:sub3}
    \end{subfigure}
   \hfill
    \begin{subfigure}[b]{0.24\textwidth}
        \includegraphics[width=\textwidth]{eccv2024/oops_radar.jpg}
        \caption{VLN-OOPS}
        \label{fig:sub4}
    \end{subfigure}

    \caption{Performance on the Re-purposed Datasets}
    \label{fig:fine_eval_radar}
\end{figure}

==> sec7-table-msrvtt.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\caption{\textbf{Performance on MSRVTT}. }
\label{tab:sec7_msr}
\centering
\scalebox{0.75}{
\begin{tabular}{llrllllllllllllllll}
\toprule
\multirow{3}{*}{Method} & \multirow{3}{*}{Traning-strategy} & \multicolumn{11}{c}{Coarse-graind Evaluation} &  & \multicolumn{5}{c}{Fine-graind Evaluation } \\
\cline{3-13} \cline{15-19}
 &  & \multicolumn{5}{c}{T2V} &  & \multicolumn{5}{c}{V2T} &  & \multirow{2}{*}{noun} & \multirow{2}{*}{adj} & \multirow{2}{*}{verb} & \multirow{2}{*}{adv} & \multirow{2}{*}{prep} \\
\cline{3-7} \cline{9-13} 
 
 &  & \multicolumn{1}{l}{R@1} & R@5 & R@10 & Med R & MeanR &  & R@1 & R@5 & R@10 & Med R & MeanR &  &  &  &  &  &  \\ \hline
\multirow{4}{*}{Frozen} & Coarse & 30.6 & \multicolumn{1}{r}{56.5} & \multicolumn{1}{r}{66.4} & \multicolumn{1}{r}{4} & \multicolumn{1}{r}{28.1} &  & \multicolumn{1}{r}{32.1} & \multicolumn{1}{r}{56.8} & \multicolumn{1}{r}{68.4} & \multicolumn{1}{r}{4} & \multicolumn{1}{r}{24.6} &  & \multicolumn{1}{r}{6.27} & \multicolumn{1}{r}{7.92} & \multicolumn{1}{r}{8.86} & \multicolumn{1}{r}{8.54} & \multicolumn{1}{r}{9.09} \\
 & Word-neg & 29.5 & \multicolumn{1}{r}{58.4} & \multicolumn{1}{r}{69.5} & \multicolumn{1}{r}{4} & \multicolumn{1}{r}{27.7} &  & \multicolumn{1}{r}{30.1} & \multicolumn{1}{r}{57.6} & \multicolumn{1}{r}{68.9} & \multicolumn{1}{r}{4} & \multicolumn{1}{r}{25.6} &  & \multicolumn{1}{r}{3.31} & \multicolumn{1}{r}{4.15} & \multicolumn{1}{r}{2.86} & \multicolumn{1}{r}{4.94} & \multicolumn{1}{r}{4.08} \\
 & Phrase-neg &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
 & Word-vpt & \multicolumn{1}{l}{} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ \hline
\multirow{4}{*}{TS2-Net} & Coarse & 46.5 & \multicolumn{1}{r}{74.0} & \multicolumn{1}{r}{81.8} & \multicolumn{1}{r}{1} & \multicolumn{1}{r}{11.5} &  & \multicolumn{1}{r}{44.2} & \multicolumn{1}{r}{72.7} & \multicolumn{1}{r}{83.1} & \multicolumn{1}{r}{2} & \multicolumn{1}{r}{9.5} &  & \multicolumn{1}{r}{5.15} & \multicolumn{1}{r}{5.84} & \multicolumn{1}{r}{7.23} & \multicolumn{1}{r}{7.82} & \multicolumn{1}{r}{8.27} \\
 & Word-neg & \multicolumn{1}{l}{} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
 & Phrase-neg &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
 & Word-vpt & \multicolumn{1}{l}{} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ \hline
\multirow{4}{*}{X-CLIP} & Coarse & 45.3 & \multicolumn{1}{r}{73.8} & \multicolumn{1}{r}{81.8} & \multicolumn{1}{r}{2.0} & \multicolumn{1}{r}{12.1} &  & \multicolumn{1}{r}{44.9} & \multicolumn{1}{r}{73.3} & \multicolumn{1}{r}{81.9} & \multicolumn{1}{r}{1} & \multicolumn{1}{r}{10.8} &  & \multicolumn{1}{r}{5.25} & \multicolumn{1}{r}{5.98} & \multicolumn{1}{r}{7.39} & \multicolumn{1}{r}{7.98} & \multicolumn{1}{r}{8.09} \\
 & Word-neg & 46.7 & \multicolumn{1}{r}{72.8} & \multicolumn{1}{r}{81.4} & \multicolumn{1}{r}{2} & \multicolumn{1}{r}{12.2} &  & \multicolumn{1}{r}{41.9} & \multicolumn{1}{r}{71.0} & \multicolumn{1}{r}{80.7} & \multicolumn{1}{r}{2} & \multicolumn{1}{r}{12.0} &  & \multicolumn{1}{r}{1.49} & \multicolumn{1}{r}{1.78} & \multicolumn{1}{r}{1.48} & \multicolumn{1}{r}{2.88} & \multicolumn{1}{r}{1.55} \\
 & Phrase-neg &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
 & Word-vpt & \multicolumn{1}{l}{} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\ \hline
\multirow{4}{*}{UCoFiA} & Coarse & 44.9 & \multicolumn{1}{r}{72.8} & \multicolumn{1}{r}{81.5} & \multicolumn{1}{r}{2.0} & \multicolumn{1}{r}{13.7} &  & \multicolumn{1}{r}{44.7} & \multicolumn{1}{r}{71.6} & \multicolumn{1}{r}{82.2} & \multicolumn{1}{r}{2} & \multicolumn{1}{r}{9.8} &  & \multicolumn{1}{r}{5.07} & \multicolumn{1}{r}{5.75} & \multicolumn{1}{r}{7.26} & \multicolumn{1}{r}{7.59} & \multicolumn{1}{r}{8.13} \\
 & Word-neg & \multicolumn{1}{l}{} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
 & Phrase-neg & \multicolumn{1}{c}{} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
 & Word-vpt & \multicolumn{1}{l}{} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\\bottomrule
\end{tabular}}
\end{table}

==> sec7-table-oops.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\caption{\textbf{Performance on OOPS}. }
\label{tab:sec7_oops}
\centering
\scalebox{0.75}{
\begin{tabular}{llrllllllllllllllll}
\toprule
\multirow{3}{*}{Method} & \multirow{3}{*}{Traning-strategy} & \multicolumn{11}{c}{Coarse-graind Evaluation} &  & \multicolumn{5}{c}{Fine-graind Evaluation } \\
\cline{3-13} \cline{15-19}
 &  & \multicolumn{5}{c}{T2V} &  & \multicolumn{5}{c}{V2T} &  & \multirow{2}{*}{noun} & \multirow{2}{*}{adj} & \multirow{2}{*}{verb} & \multirow{2}{*}{adv} & \multirow{2}{*}{prep} \\
\cline{3-7} \cline{9-13} 
 
 &  & \multicolumn{1}{l}{R@1} & R@5 & R@10 & Med R & MeanR &  & R@1 & R@5 & R@10 & Med R & MeanR &  &  &  &  &  &  \\ \hline
\multirow{4}{*}{Frozen} & Coarse & 29.7 & 57.0 & 67.7 & 4 & 52.1 &  & 30.6 & 57.3 & 67.9 & 4 & 44.6 &  & \multicolumn{1}{r}{6.52} & \multicolumn{1}{r}{7.33} & \multicolumn{1}{r}{9.77} & \multicolumn{1}{r}{9.48} & \multicolumn{1}{r}{9.10} \\
 & Word-neg & 28.6 & 56.1 & 65.0 & 4 & 55.3 &  & 27.2 & 53.5 & 65.6 & 5 & 45.5 &  & \multicolumn{1}{r}{2.34} & \multicolumn{1}{r}{2.35} & \multicolumn{1}{r}{1.61} & \multicolumn{1}{r}{3.27} & \multicolumn{1}{r}{2.53} \\
 & Phrase-neg &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  &  &  &  &  &  \\
 & Word-vpt & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  &  &  &  &  &  \\ \hline
\multirow{4}{*}{TS2-Net} & Coarse & 31.6 & 57.5 & 66.4 & 4 & 56.2 &  & 45.6 & 74.4 & 83.6 & 2 & 14.7 &  & \multicolumn{1}{r}{5.47} & \multicolumn{1}{r}{5.94} & \multicolumn{1}{r}{9.45} & \multicolumn{1}{r}{11.20} & \multicolumn{1}{r}{9.79} \\
 & Word-neg & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  &  &  &  &  &  \\
 & Phrase-neg &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  &  &  &  &  &  \\
 & Word-vpt & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  &  &  &  &  &  \\ \hline
\multirow{4}{*}{X-CLIP} & Coarse & 32.3 & 57.8 & 66.7 & 3 & 49.5 &  & 46.3 & 77.9 & 86.1 & 2 & 11.2 &  & \multicolumn{1}{r}{5.78} & \multicolumn{1}{r}{6.11} & \multicolumn{1}{r}{9.40} & \multicolumn{1}{r}{11.36} & \multicolumn{1}{r}{9.89} \\
 & Word-neg & 31.5 & 56.5 & 65.4 & 4 & 55.6 &  & 40.2 & 69.4 & 79.1 & 2 & 19.9 &  & \multicolumn{1}{r}{1.31} & \multicolumn{1}{r}{1.51} & \multicolumn{1}{r}{1.08} & \multicolumn{1}{r}{5.01} & \multicolumn{1}{r}{2.61} \\
 & Phrase-neg & 31.4 & 56.8 & 66.2 & 4 & 54.8 &  & 44.5 & 74.3 & 82.6 & 2 & 16.7 &  &  &  &  &  &  \\
 & Word-vpt & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  &  &  &  &  &  \\ \hline
\multirow{4}{*}{UCoFiA} & Coarse & 30.2 & 56.2 & 65.4 & 4 & 57.9 &  & 43.0 & 73.0 & 82.7 & 2 & 14.0 &  & \multicolumn{1}{r}{5.00} & \multicolumn{1}{r}{6.33} & \multicolumn{1}{r}{8.82} & \multicolumn{1}{r}{11.26} & \multicolumn{1}{r}{9.81} \\
 & Word-neg & 30.8 & 55.9 & 64.8 & 4 & 52.3 &  & 38.4 & 66.2 & 76.6 & 2 & 20.6 &  & \multicolumn{1}{r}{1.24} & \multicolumn{1}{r}{1.45} & \multicolumn{1}{r}{1.06} & \multicolumn{1}{r}{4.83} & \multicolumn{1}{r}{2.56} \\
 & Phrase-neg & 30.0 & 55.8 & 65.3 & 4 & 57.4 &  & 36.5 & 67.3 & 78.1 & 2 & 23.1 &  & \multicolumn{1}{r}{1.29} & \multicolumn{1}{r}{1.98} & \multicolumn{1}{r}{1.32} & \multicolumn{1}{r}{5.98} & \multicolumn{1}{r}{3.74} \\
 & Word-vpt & \multicolumn{1}{l}{} &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\\bottomrule
\end{tabular}}
\end{table}

==> sec7-table-vatex.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\caption{\textbf{Performance on VATEX}. }
\label{tab:sec7_vatex}
\centering
\scalebox{0.75}{
\begin{tabular}{llrllllllllllllllll}
\toprule
\multirow{3}{*}{Method} & \multirow{3}{*}{Traning-strategy} & \multicolumn{11}{c}{Coarse-graind Evaluation} &  & \multicolumn{5}{c}{Fine-graind Evaluation } \\
\cline{3-13} \cline{15-19}
 &  & \multicolumn{5}{c}{T2V} &  & \multicolumn{5}{c}{V2T} &  & \multirow{2}{*}{noun} & \multirow{2}{*}{adj} & \multirow{2}{*}{verb} & \multirow{2}{*}{adv} & \multirow{2}{*}{prep} \\
\cline{3-7} \cline{9-13} 
 
 &  & \multicolumn{1}{l}{R@1} & R@5 & R@10 & Med R & MeanR &  & R@1 & R@5 & R@10 & Med R & MeanR &  &  &  &  &  &  \\ \hline
\multirow{4}{*}{Frozen} & Coarse & 41.7 & 77.7 & 88.2 & 2 & 7.5 &  & 40.8 & 79.2 & 88.0 & 2 & 7.7 &  & \multicolumn{1}{r}{6.99} & \multicolumn{1}{r}{7.79} & \multicolumn{1}{r}{8.47} & \multicolumn{1}{r}{9.72} & \multicolumn{1}{r}{9.76} \\
 & Word-neg & 42.4 & 78.9 & 87.3 & 2 & 7.6 &  & 38.5 & 73.5 & 84.3 & 2 & 10.1 &  & \multicolumn{1}{r}{2.32} & \multicolumn{1}{r}{2.80} & \multicolumn{1}{r}{1.80} & \multicolumn{1}{r}{4.02} & \multicolumn{1}{r}{2.10} \\
 & Phrase-neg &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  &  &  &  &  &  \\
 & Word-vpt & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  &  &  &  &  &  \\ \hline
\multirow{4}{*}{TS2-Net} & Coarse & 61.1 & 90.9 & 95.7 & 1 & 3.2 &  & 77.2 & 97.2 & 98.8 & 1 & 1.6 &  & \multicolumn{1}{r}{6.69} & \multicolumn{1}{r}{7.20} & \multicolumn{1}{r}{8.68} & \multicolumn{1}{r}{8.24} & \multicolumn{1}{r}{9.46} \\
 & Word-neg & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  &  &  &  &  &  \\
 & Phrase-neg &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  &  &  &  &  &  \\
 & Word-vpt & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  &  &  &  &  &  \\ \hline
\multirow{4}{*}{X-CLIP} & Coarse & 61.7 & 90.3 & 95.0 & 1 & 3.6 &  & 77.2 & 97.2 & 98.8 & 1 & 1.6 &  & \multicolumn{1}{r}{6.94} & \multicolumn{1}{r}{7.20} & \multicolumn{1}{r}{8.53} & \multicolumn{1}{r}{8.69} & \multicolumn{1}{r}{9.64} \\
 & Word-neg & 55.2 & 86.8 & 92.5 & 1 & 16.2 &  & 63.4 & 94.4 & 98.0 & 1 & 2.2 &  &  &  &  &  &  \\
 & Phrase-neg & 56.5 & 87.6 & 93.7 & 1 & 12.1 &  & 66.4 & 94.9 & 98.4 & 1 & 2.0 &  &  &  &  &  &  \\
 & Word-vpt & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  &  &  &  &  &  \\ \hline
\multirow{4}{*}{UCoFiA} & Coarse & 59.9 & 89.2 & 94.6 & 1 & 3.8 &  & 73.6 & 95.8 & 98.3 & 1 & 2.0 &  & \multicolumn{1}{r}{7.66} & \multicolumn{1}{r}{7.96} & \multicolumn{1}{r}{8.98} & \multicolumn{1}{r}{8.87} & \multicolumn{1}{r}{10.10} \\
 & Word-neg & 59.9 & 90.1 & 95.1 & 1 & 3.4 &  & 68.3 & 96.0 & 98.6 & 1 & 1.9 &  & \multicolumn{1}{r}{1.56} & \multicolumn{1}{r}{1.69} & \multicolumn{1}{r}{1.48} & \multicolumn{1}{r}{2.19} & \multicolumn{1}{r}{2.32} \\
 & Phrase-neg & 60.5 & 90.1 & 95.0 & 1 & 3.4 &  & 73.7 & 97.4 & 99.0 & 1 & 1.7 &  & \multicolumn{1}{r}{1.77} & \multicolumn{1}{r}{2.33} & \multicolumn{1}{r}{1.99} & \multicolumn{1}{r}{2.83} & \multicolumn{1}{r}{3.41} \\
 & Word-vpt & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  &  &  &  &  &  \\ \hline
\\\bottomrule
\end{tabular}}
\end{table}

==> tab-ablation-N.tex <==

\begin{table}[t]
\caption{\textbf{Number of hard negative sentences $\mathbb{N}$}. With $\mathbb{N}=16$, the model maintains robust performance and improves in fine-grained metrics.}
\vspace{-0.8em}
\label{tab:ablation1}
\centering
\setlength{\tabcolsep}{2pt}
\resizebox{0.5\linewidth}{!}{
\begin{tabular}{llccccccc}
\toprule
\multirow{2}{*}{$\mathbb{N}$}  & \multicolumn{2}{c}{Coarse-Grained ($\uparrow$)} &  & \multicolumn{5}{c}{Fine-Grained ($\downarrow$)} \\
\cmidrule{2-3} \cmidrule{5-9}
 & \multirow{1}{*}{V2T}  &  \multirow{1}{*}{T2V} & & \multirow{1}{*}{noun} & \multirow{1}{*}{adj} & \multirow{1}{*}{verb} & \multirow{1}{*}{adv} & \multirow{1}{*}{prep} \\
 \midrule
2 & 53.3 & 39.9 &  & 1.83 & 2.59 & 1.50 & 8.61 & 3.78 \\
4 & 48.6 & 39.8 &  & 1.36 & 1.67 & 1.12 & 7.27 & 2.35 \\
8 & 48.7 & 39.8 &  & 1.38 & 1.57 & 1.11 & 6.33 & 2.56 \\
16 & 47.5 & 40.0 &  & 1.30 & 1.41 & 1.09 & 5.49 & 2.28 \\
32 & 44.0 & 40.0 &  & 1.26 & 1.37 & 1.06 & 5.88 & 2.15 \\
 %& Word-vpt & 19.2 & 41.6 & 54.2 &  & 19.3 & 44.2 & 56.7 &  &  &  &  &  &  \\
 \bottomrule
\end{tabular}}
\vspace{6em}
\end{table}






% \begin{table}[]
% \setlength{\tabcolsep}{3pt}

% \caption{\textbf{Number of hard negative sentences $\mathbb{N}$}. }
% \label{tab:ablation1}
% \centering
% \scalebox{0.75}{
% \begin{tabular}{lrrrrrrrrrrrrr}
% \toprule
%  \multirow{3}{*}{$\mathbb{N}$} & \multicolumn{7}{c}{Coarse-Grained Evaluation ($\uparrow$)} &  & \multicolumn{5}{c}{Fine-Grained Evaluation ($\downarrow$)} \\
% \cmidrule{2-8} \cmidrule{10-14}
% & \multicolumn{3}{c}{\multirow{1}{*}{T2V}} &  & \multicolumn{3}{c}{\multirow{1}{*}{V2T}} &  & \multirow{2}{*}{noun} & \multirow{2}{*}{adj} & \multirow{2}{*}{verb} & \multirow{2}{*}{adv} & \multirow{2}{*}{prep} \\
% \cmidrule{2-4} \cmidrule{6-8}
% & \multirow{1}{*}{R@1} & \multirow{1}{*}{R@5} & \multirow{1}{*}{R@10} &  & \multirow{1}{*}{R@1} & \multirow{1}{*}{R@5} & \multirow{1}{*}{R@10} \\ \midrule
% \multicolumn{1}{c}{2} & 21.8	&43.5& 	54.3  &   & 29.8	&59.2&	70.9  &  &1.83&  2.59& 1.50 & 8.61&  3.78 \\
% \multicolumn{1}{c}{4} &21.7	  &43.3	  &54.3  &  &26.0	 &53.1	  &66.6  &  & 1.36& 1.67 & 1.12 & 7.27 & 2.35 \\
% \multicolumn{1}{c}{8} & 21.9 &  43.6 & 53.8 &  & 26.1 & 53.4 & 66.5   &  & 1.38& 1.57& 1.11  & 6.33& 2.56   \\
% \multicolumn{1}{c}{16} & 21.9 & 43.9 & 54.2 &  & 24.9 & 52.6 & 64.9 &  & 1.30 & 1.41 & 1.09 & 5.49 & 2.28  \\
% \multicolumn{1}{c}{32} &21.6	  &43.8	  &54.6  &  &22.7	  &48.3	  &61.1  &  & 1.26& 1.37 & 1.06 & 5.88 &  2.15 \\ \bottomrule
% \end{tabular}}
% \end{table}

==> tab-ablation-T.tex <==

% \begin{table}[t]
% \caption{\textbf{Number of visual prompts (VPs) $\mathbb{T}$}. }
% \vspace{-0.8em}
% \label{tab:ablation3}
% \centering
% \setlength{\tabcolsep}{2pt}
% \resizebox{0.5\linewidth}{!}{
% \begin{tabular}{llccccccc}
% \toprule
% \multirow{2}{*}{$\mathbb{T}$}  & \multicolumn{2}{c}{Coarse-Grained ($\uparrow$)} &  & \multicolumn{5}{c}{Fine-Grained ($\downarrow$)} \\
% \cmidrule{2-3} \cmidrule{5-9}
%  & \multirow{1}{*}{V2T}  &  \multirow{1}{*}{T2V} & & \multirow{1}{*}{noun} & \multirow{1}{*}{adj} & \multirow{1}{*}{verb} & \multirow{1}{*}{adv} & \multirow{1}{*}{prep} \\
%  \midrule
% 0 & 47.5 & 40.0 &  & 1.30 & 1.41 & 1.09 & 5.49 & 2.28 \\
% 1 & 53.1 & 39.3 &  & 1.38 & 1.48 & 1.12 & 5.15 & 2.33 \\
% 2 & 54.0 & 39.8 &  & 1.39 & 1.67 & 1.13 & 6.18 & 3.23 \\
% 4 & 54.0 & 40.2 &  & 1.38 & 1.66 & 1.14 & 6.15 & 3.42 \\
% 8 & 52.5 & 39.7 &  & 1.42 & 1.74 & 1.13 & 6.28 & 3.35 \\
%  %& Word-vpt & 19.2 & 41.6 & 54.2 &  & 19.3 & 44.2 & 56.7 &  &  &  &  &  &  \\
%  \bottomrule
% \end{tabular}}
% \vspace{-0.5em}
% \end{table}




% \begin{table}[]
% \caption{\textbf{Number of visual prompts (VPs) $\mathbb{T}$}. }
% \setlength{\tabcolsep}{3pt}
% \label{tab:ablation3}
% \centering
% \scalebox{0.75}{
% \begin{tabular}{lrllllllllllll}
% \toprule
%  \multirow{3}{*}{$\mathbb{T}$} & \multicolumn{7}{c}{Coarse-Grained Evaluation ($\uparrow$)} &  & \multicolumn{5}{c}{Fine-Grained Evaluation ($\downarrow$)} \\
% \cmidrule{2-8} \cmidrule{10-14}
%  & \multicolumn{3}{c}{\multirow{1}{*}{T2V}} &  & \multicolumn{3}{c}{\multirow{1}{*}{V2T}} &  & \multirow{2}{*}{noun} & \multirow{2}{*}{adj} & \multirow{2}{*}{verb} & \multirow{2}{*}{adv} & \multirow{2}{*}{prep} \\
% \cmidrule{2-4} \cmidrule{6-8}
%  & \multirow{1}{*}{R@1} & \multirow{1}{*}{R@5} & \multirow{1}{*}{R@10} &  & \multirow{1}{*}{R@1} & \multirow{1}{*}{R@5} & \multirow{1}{*}{R@10} &  &   \\ \midrule
%  \multicolumn{1}{c}{0} & 21.9 & 43.9 & 54.2 &  & 24.9 & 52.6 & 64.9 &  & 1.30 & 1.41 & 1.09 & 5.49 & 2.28  \\
% \multicolumn{1}{c}{1} &21.5  &42.4	& 53.9   &  &30.1	 &58.4	  &70.7   & &1.38	&1.48	 &1.12		 &5.15	 &2.33    \\
% \multicolumn{1}{c}{2} & 21.4	 & 43.4& 	54.5  &  & 30.3	&59.6 & 	72.1   &  & 1.39 &	1.67	& 1.13	& 6.18	 &3.23    \\
% \multicolumn{1}{c}{4} &22.3	&43.6	&54.7     &  &30.7	&60.0	&71.3    &  &1.38		&1.66   &1.14	 &6.15		  & 3.42 \\
% \multicolumn{1}{c}{8} & 21.5& 	43.3	&54.2    &  & 29.3	 & 57.9	&70.3   &  & 1.42	&1.74	&1.13	 &6.28&	3.35        \\
%  \bottomrule
% \end{tabular}}
% \end{table}

 \vspace{-2em}
\begin{wraptable}{r}{0.38\textwidth} % 表格将位于页面的右侧，占据大约一半的文本宽度
\vspace{-2.5em}
\caption{\textbf{Number of visual prompts $\mathbb{T}$}.  $\mathbb{T}{=}1$ balances  performance and training efficiency. }
% \vspace{-0.8em}
\label{tab:ablation3}
\centering
\setlength{\tabcolsep}{2pt}
\resizebox{\linewidth}{!}{ % 注意这里的 \linewidth 是 wraptable 环境的宽度
\begin{tabular}{llccccccc}
\toprule
\multirow{2}{*}{$\mathbb{T}$} & \multicolumn{2}{c}{Coarse-Grained ($\uparrow$)} && \multicolumn{5}{c}{Fine-Grained ($\downarrow$)} \\
\cmidrule{2-3} \cmidrule{5-9}
& \multirow{1}{*}{V2T} & \multirow{1}{*}{T2V} && \multirow{1}{*}{noun} & \multirow{1}{*}{adj} & \multirow{1}{*}{verb} & \multirow{1}{*}{adv} & \multirow{1}{*}{prep} \\
\midrule
0 & 47.5 & 40.0 && 1.30 & 1.41 & 1.09 & 5.49 & 2.28 \\
1 & 53.1 & 39.3 && 1.38 & 1.48 & 1.12 & 5.15 & 2.33 \\
2 & 54.0 & 39.8 && 1.39 & 1.67 & 1.13 & 6.18 & 3.23 \\
4 & 54.0 & 40.2 && 1.38 & 1.66 & 1.14 & 6.15 & 3.42 \\
8 & 52.5 & 39.7 && 1.42 & 1.74 & 1.13 & 6.28 & 3.35 \\
\bottomrule
\end{tabular}}
\vspace{-2em}
\end{wraptable}

==> tab-ablation-lambda.tex <==

\begin{table}[t]
\caption{\textbf{Loss weight $\lambda$}. $\lambda{=}0.2$ is the best balance between fine-grained and coarse-grained performances. }
\vspace{-0.8em}
\label{tab:ablation2}
\centering
\setlength{\tabcolsep}{2pt}
\resizebox{0.5\linewidth}{!}{
\begin{tabular}{llccccccc}
\toprule
\multirow{2}{*}{$\lambda$}  & \multicolumn{2}{c}{Coarse-Grained ($\uparrow$)} &  & \multicolumn{5}{c}{Fine-Grained ($\downarrow$)} \\
\cmidrule{2-3} \cmidrule{5-9}
 & \multirow{1}{*}{V2T}  &  \multirow{1}{*}{T2V} & & \multirow{1}{*}{noun} & \multirow{1}{*}{adj} & \multirow{1}{*}{verb} & \multirow{1}{*}{adv} & \multirow{1}{*}{prep} \\
 \midrule
0.1 & 48.2 & 39.8 &  & 1.39 & 1.67 & 1.12 & 6.99 & 2.54 \\
0.2 & 47.5 & 40.0 &  & 1.30 & 1.41 & 1.09 & 5.49 & 2.28 \\
0.3 & 42.7 & 40.0 &  & 1.26 & 1.30 & 1.06 & 5.68 & 2.12 \\
0.4 & 41.4 & 39.5 &  & 1.24 & 1.32 & 1.05 & 5.47 & 2.07 \\
0.5 & 43.3 & 39.4 &  & 1.25 & 1.33 & 1.06 & 4.99 & 2.16 \\
 %& Word-vpt & 19.2 & 41.6 & 54.2 &  & 19.3 & 44.2 & 56.7 &  &  &  &  &  &  \\
 \bottomrule
\end{tabular}}
\vspace{-0.8em}
\end{table}





% \begin{table}[]
% \caption{\textbf{Loss weight $\lambda$}. }
% \label{tab:ablation2}
% \setlength{\tabcolsep}{3pt}
% \centering
% \scalebox{0.75}{
% \begin{tabular}{lrrrrrrrrrrrrr}
% \toprule
%  \multirow{3}{*}{ $\lambda$ } & \multicolumn{7}{c}{Coarse-Grained Evaluation ($\uparrow$)} &  & \multicolumn{5}{c}{Fine-Grained Evaluation ($\downarrow$)} \\
% \cmidrule{2-8} \cmidrule{10-14}
%   & \multicolumn{3}{c}{\multirow{1}{*}{T2V}} &  & \multicolumn{3}{c}{\multirow{1}{*}{V2T}} &  & \multirow{2}{*}{noun} & \multirow{2}{*}{adj} & \multirow{2}{*}{verb} & \multirow{2}{*}{adv} & \multirow{2}{*}{prep} \\
% \cmidrule{2-4} \cmidrule{6-8}
%    & \multirow{1}{*}{R@1} & \multirow{1}{*}{R@5} & \multirow{1}{*}{R@10} &  & \multirow{1}{*}{R@1} & \multirow{1}{*}{R@5} & \multirow{1}{*}{R@10} &  &   \\ \midrule
%  \multicolumn{1}{c}{0.1} &21.4	  &43.2	  &54.8  &  &26.1	  &52.3	  &66.3  &  &1.39 	& 1.67	&1.12	 & 6.99	& 2.54    \\
%  \multicolumn{1}{c}{0.2} & 21.9 & 43.9 & 54.2 &  & 24.9 & 52.6 & 64.9 &  & 1.30 & 1.41 & 1.09 & 5.49 & 2.28  \\
%  \multicolumn{1}{c}{0.3} &21.7	  &43.4	  &54.8  &  &21.7	 &46.6	   &59.7  &  &  1.26	& 1.30	&1.06 &	5.68	&2.12      \\
%  \multicolumn{1}{c}{0.4} &21.7	  &42.9	  &54.0  &  &21.2	  &45.2	  &57.7  &  &  1.24	& 1.32&	1.05	&5.47 & 	2.07     \\
%  \multicolumn{1}{c}{0.5} & 21.6	& 42.7	&53.9 &  &  21.7& 47.5&  60.6 &  & 1.25 & 1.33 & 1.06 & 4.99& 2.16  \\
%  \bottomrule
% \end{tabular}}
% \end{table}

==> tab-dataset.tex <==
\begin{table}[t]
\caption{\textbf{Details of Benchmarks in Text-to-Video Retrieval}. We show the number of videos and captions in the train and test sets alongside the size of the vocabularly for nouns, verbs, adjectives, adverbs and prepositions.}
\vspace{-1em}
\label{tab:benchmarks}
\resizebox{\linewidth}{!}{
\begin{tabular}{lrrrrrrrrrrrrrrrc}
\midrule
  & & &\multicolumn{2}{c}{Training Set} & & \multicolumn{2}{c}{Test Set} & & \multicolumn{6}{c}{Vocabulary} \\
  \cmidrule{4-5} \cmidrule{7-8} \cmidrule{10-15}
\multicolumn{1}{l}{\multirow{-2}{*}{Dataset}} & \multirow{1}{*}{Source}&  & \#Video & \multicolumn{1}{c}{\multirow{1}{*}{\#Caption}} & & \multicolumn{1}{c}{\#Video} & \multicolumn{1}{c}{\#Caption} & & All & \multicolumn{1}{c}{Noun} & \multicolumn{1}{c}{Verb} & \multicolumn{1}{c}{Adj} & \multicolumn{1}{c}{Adv} & \multicolumn{1}{c}{Prep}  & & Eval. Metrics\\ \midrule 
YouCook2 \cite{Zhou2018youcook2} & YouTube &&13.8k& 13.8k &  & 3.3K & 3.3k & & 2,266  & 1,495 & 668 & 447 & 97 & 8 && Recall@k, Av. Rank\\
DiDeMo \cite{didemo} & Flicker& & 10.6K& 41.2k &  & 1.0K & 4.0k & & 6,763 &  4,401 & 2,404 & 889 & 279 & 23 && Recall@k \\
ActivityNet \cite{activitynetcap} & YouTube& & 10.9K& 10.9k & & 4.9k & 4.9k & & 12,959  & 8,021 & 4,824 & 1,927 & 545 & 91 & & Recall@k \\
VATEX \cite{wang2019vatex} &  YouTube & &28.9k&  289.9k & & 1.5k & 15.0k & & 29,065 &  18,247 & 10,606 & 5,092 & 1,259 & 173  & & Recall@k, Av. Rank\\
MSVD  \cite{chen2011msvd} & YouTube && 1.3k& 52.9k & & 670 & 27.8k & & 12,926  & 7,763 & 4,401 & 1,788 & 425 & 89  & & Recall@k, Av. Rank\\
TGIF \cite{tgif2015} & Tumblr && 89.4k& 90.4k &  & 11.3k  & 34.1k & & 11,438 &  6,809 & 4,432 & 1,832 & 585 & 37 &&Recall@k, Av. Rank \\
MSR-VTT \cite{xu2016msr} & YouTube &&9k & 180k & & 1,000 & 1k & & 25,692  & 16,719 & 8,007 & 4,380 & 929 & 105   & & Recall@k, Av. Rank\\
%OPS & caption & Open & YouTube & 32k & 4,877 & 2,047 & 5.4k & 3,163 & 1,718 & 624 & 192 & 24 \\
%UVO & caption & Open & YouTube & 19k & 3,669 & 2,707 & 6.6k & 2,489 & 1,146 & 448 & 74 & 14 \\ 
\bottomrule
\end{tabular}
}
\vspace{-0.9em}
\end{table}

% \begin{table}[tbh!]
%  \resizebox{\linewidth}{!}{
%  \begin{tabular}{llllrrrrrrrrr}
%  \caption{\textbf{Details of benchmarks in Text-to-Video Retrieval}. }
%  \label{tab:benchmarks}
%   \hline
%   & \multicolumn{1}{l}{}& \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{}  & \multicolumn{1}{l}{} &\multicolumn{2}{c}{Test set}& \multicolumn{5}{c}{Part of speech} \\
%   \multirow{-2}{*}{Dataset} & \multicolumn{1}{l}{\multirow{-2}{*}{Text type}} & \multicolumn{1}{l}{\multirow{-2}{*}{Scenario}} & \multicolumn{1}{l}{\multirow{-2}{*}{Source}} & \multicolumn{1}{l}{\multirow{-2}{*}{\#Sentences}} & \multicolumn{1}{l}{\multirow{-2}{*}{\#vocab}} & \multicolumn{1}{l}{\#Video} & \multicolumn{1}{l}{\#Sentence} & \multicolumn{1}{l}{Noun} & \multicolumn{1}{l}{Verb} & \multicolumn{1}{l}{Adjective} & \multicolumn{1}{l}{Adverb} & \multicolumn{1}{l}{Adposition}  \\
%   \midrule
%   MSVD     & caption    & Open   & You-Tube    & 81k    & 12,926     & 670 & 27.8k   & 7,763 & 4,401 & 1,788 & 425 & 89 \\
%   % LSMDC  & paragraph & Movie Scripts& Movies & 118k  & \multicolumn{1}{l}{}  & 1,000   & 1.0k  & \multicolumn{1}{l}{}  &\multicolumn{1}{l}{}     & \multicolumn{1}{l}{}& \multicolumn{1}{l}{}& \multicolumn{1}{l}{}     \\
%   DiDeMo  & paragraph & Open  & Flicker video  & 40k& 6,763 & 1,004& 4.0k & 4,401 & 2,404 & 889 & 279 & 23 \\
%   VATEX& caption & Open &You-Tube   & 256k  & 29,065   & 1,500 & 15.0k & 18,247 & 10,606 & 5,092 & 1,259 & 173 \\
%   MSR-VTT  & caption  & Open  & You-Tube & 200k  & 25,692& 2,990 & 59.8k & 16,719 & 8,007 & 4,380 & 929 & 105 \\
%   You-cook2& caption   & Cooking & You-Tube & 15k  & 2,266  & 457  & 3.5k   & 1,495 & 668 & 447 & 97 & 8 \\
%   ActivityNet-cap  & paragraph  & Daily Living  & You-Tube & 20k & 12,959  & 4,917  & 4.9k & 8,021 & 4,824 & 1,927 & 545 & 91 \\
%   TGIF & caption  & Open & Tumblr GIFs  & 125k  & \multicolumn{1}{l}{} & 11,351 & 34.1k & \multicolumn{1}{l}{} & \multicolumn{1}{l}{}& \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{}    \\
%   \multicolumn{14}{l}{Reorganized existing datasets}  \\
%   Oops & caption& Open& You-Tube& 32k  & 4,877 & 2,047 &5.4k&3,163 & 1,718 & 624 & 192 & 24 \\
%   UVO & caption & Open  & YouTube & 19k & 3,669& 2,707 & 6.6k &2,489 & 1,146 & 448 & 74 & 14  \\ \bottomrule    
%  \end{tabular}}
% \end{table}


% % \begin{table}[tbh!]
% % \centering
% % \setlength{\abovecaptionskip}{0.cm}
% % \setlength{\belowcaptionskip}{-0.cm}
% % \normalsize
% % \caption{\textbf{Details of benchmarks in Text-to-Video Retrieval}. }
% % \label{tab:benchmarks}
% % \begin{center}
% % \scalebox{0.7}{
% % \begin{tabular}{llllrrrrrrrrrr}
% % \hline

% % \multirow{2}{*}{\textbf{Dataset}}
% % &\multirow{2}{*}{\textbf{Text Type}} &\multirow{2}{*}{\textbf{Scenario}} &\multirow{2}{*}{\textbf{Source}} &\multirow{2}{*}{\textbf{#Sentences}} &\multirow{2}{*}{\textbf{#Vocab-size}}  &\multicolumn{2}{c}{\textbf{Test set size}}   &\multicolumn{5}{c}{\textbf{Part-of-speech }}  \\
% % \cline{7-8}  \cline{8-14} 
% % && &\textit{#Video} & \textit{#Sentence} &\textit{Noun} & \textit{Verb} &\textit{ADJ} & \textit{ADV}  & \textit{ADP}\\
% % \hline
% % % IACC.3 & 335,944 & 3,845,221 & 
% % % \multicolumn{1}{c}{TV16: 30, TV17: 30, TV18: 30}   
% % % & \multicolumn{1}{c}{7.8}  & \multicolumn{1}{c}{2.2}  \\ \hline
% % % V3C1  & 1,082,649 & 7,839,450 &\multicolumn{1}{c}{TV19: 30, TV20: 30, TV21: 20}   &\multicolumn{1}{c}{3.3}  &\multicolumn{1}{c}{1.2} \\\hline
% % \end{tabular}

% % }
% % \end{center}
% % \end{table}
% % V3C2  & 1,425,443 & 10,192,839 & 20   & 3.3  & 1.2  \\ \hline
% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% % \usepackage[table,xcdraw]{xcolor}
% % Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
% % \usepackage[normalem]{ulem}
% % \useunder{\uline}{\ul}{}


==> tab-fine_data.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\caption{\textbf{Public datasets re-purposed by this paper for fine-grained evaluation}.}
\label{tab:fine_data}
\centering
\begin{tabular}{lrrrrrrrrrr}
 \hline
\multirow{2}{*}{Dataset} & \multicolumn{2}{c}{\textit{noun}} & \multicolumn{2}{c}{\textit{verb}} & \multicolumn{2}{c}{\textit{adj}} & \multicolumn{2}{c}{\textit{adv}} & \multicolumn{2}{c}{\textit{prep}} \\
 & \multicolumn{1}{c}{video} & \multicolumn{1}{c}{sent} & \multicolumn{1}{c}{video} & \multicolumn{1}{c}{sent} & \multicolumn{1}{c}{video} & \multicolumn{1}{c}{sent} & \multicolumn{1}{c}{video} & \multicolumn{1}{c}{sent} & \multicolumn{1}{c}{video} & \multicolumn{1}{c}{sent} \\ \hline
VATEX & 1,397 & 13,969 & 1,397 & 13,495 & 1,371 & 6,409 & 832 & 1,542 & 450 & 577 \\
MSR-VTT & 1,000 & 19,911 & 1,000 & 1,750 & 963 & 6,470 & 428 & 814 & 248 & 405 \\
VLN-UVO & 2,663 & 6,559 & 2,659 & 6,499 & 2,583 & 5,725 & 190 & 218 & 180 & 236 \\
VLN-OOPS & 1,964 & 5,335 & 1,964 & 5,315 & 1,911 & 4,729 & 673 & 886 & 239 & 304  \\ \hline
\end{tabular}
\end{table}

==> tab-fine_eval.tex <==

% \usepackage{multirow}
% \begin{table}[tb]
% \caption{\textbf{Performance on the re-purposed Datasets}. We retrained the aforementioned four models, keeping all hyper-parameters consistent with the original settings except for the batch size, which we set to 256 in our experiments.}
% \label{tab:fine_grained_evaluation}
%  \centering
% \begin{tabular}{llrrrrr}
% \hline
% Dataset & Method & \multicolumn{1}{l}{Noun} & \multicolumn{1}{l}{ADJ} & \multicolumn{1}{l}{Verb} & \multicolumn{1}{l}{ADV} & \multicolumn{1}{l}{ADP} \\ \hline
% \multirow{4}{*}{MSR-VTT} & Frozen & 6.27 & 7.92 & 8.86 & 8.54 & 9.09 \\ 
%  & TS2-Net & 5.15 & 5.84 & 7.23 & 7.82 & 8.27 \\
%  & X-CLIP & 5.25 & 7.98 & 7.39 & 5.25 & 4.50 \\
%  & UCoFiA & 5.07 & 5.75 & 7.26 & 7.59 & 8.13 \\ \hline
% \multirow{4}{*}{VATEX} & Frozen & 6.99 & 7.79 & 8.47 & 9.72 & 9.76 \\
%  & TS2-Net & 6.69 & 7.20 & 8.68 & 8.24 & 9.46 \\
%  & X-CLIP & 6.94 & 7.20 & 8.53 & 8.69 & 9.64 \\
%  & UCoFiA & 7.66 & 7.96 & 8.98 & 8.87 & 10.10 \\ \hline
% \multirow{4}{*}{VLN-UVO} & Frozen & 6.61 & 7.22 & 9.06 & 9.08 & 8.88 \\
%  & TS2-Net & 6.00 & 6.00 & 7.06 & 10.18 & 8.64 \\
%  & X-CLIP & 5.99 & 6.08 & 7.16 & 10.60 & 8.51 \\
%  & UCoFiA & 5.69 & 6.21 & 7.16 & 10.31 & 8.43 \\ \hline
% \multirow{4}{*}{VLN-OOPS} & Frozen & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
%  & TS2-Net & 5.47 & 5.94 & 9.45 & 11.20 & 9.79 \\
%  & X-CLIP & 5.78 & 6.11 & 9.40 & 11.36 & 9.89 \\
%  & UCoFiA & 5.00 & 6.33 & 8.82 & 11.26 & 9.81 \\ \hline
% \end{tabular}
% \end{table}





% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\caption{\textbf{Performance on the re-purposed Datasets}. The following four models were retrained, with all hyper-parameters consistent with the original settings except for the batch size, which was set to $256$ in the experiments. \textbf{Metric: \textit{FmR ($\downarrow$})}}
\label{tab:fine_grained_evaluation}
\centering
\scalebox{0.75}{
\begin{tabular}{llrrrrrlrrrrrlrrrrrlrrrrr}
 \hline
\multirow{2}{*}{Model} &  & \multicolumn{5}{c}{MSR-VTT} &  & \multicolumn{5}{c}{VATEX} &  & \multicolumn{5}{c}{VLN-UVO} &  & \multicolumn{5}{c}{VLN-OOPS} \\
\cline{3-7} \cline{9-13} \cline{15-19} \cline{21-25}
 &  & \multicolumn{1}{l}{\textit{noun}} & \multicolumn{1}{l}{\textit{adj}} & \multicolumn{1}{l}{\textit{verb}} & \multicolumn{1}{l}{\textit{adv}} & \multicolumn{1}{l}{\textit{prep}} &  & \multicolumn{1}{l}{\textit{noun}} & \multicolumn{1}{l}{\textit{adj}} & \multicolumn{1}{l}{\textit{verb}} & \multicolumn{1}{l}{\textit{adv}} & \multicolumn{1}{l}{\textit{prep}} &  & \multicolumn{1}{l}{\textit{noun}} & \multicolumn{1}{l}{\textit{adj}} & \multicolumn{1}{l}{\textit{verb}} & \multicolumn{1}{l}{\textit{adv}} & \multicolumn{1}{l}{\textit{prep}} &  & \multicolumn{1}{l}{\textit{noun}} & \multicolumn{1}{l}{\textit{adj}} & \multicolumn{1}{l}{\textit{verb}} & \multicolumn{1}{l}{\textit{adv}} & \multicolumn{1}{l}{\textit{prep}} \\  \hline
Frozen &  & 6.27 & 7.92 & 8.86 & 8.54 & 9.09 &  & 6.99 & 7.79 & 8.47 & 9.72 & 9.76 &  & 6.61 & 7.22 & 9.06 & 9.08 & 8.88 & & 6.52 & 7.33 & 9.77 & 9.48 & 9.10 \\   
TS2-Net &  & 5.15 & 5.84 & 7.23 & 7.82 & 8.27 &  & 6.69 & 7.20 & 8.68 & 8.24 & 9.46 &  & 6.00 & 6.00 & 7.06 & 10.18 & 8.64 &  & 5.47 & 5.94 & 9.45 & 11.20 & 9.79 \\
X-CLIP &  & 5.25 & 5.98 & 7.39 & 7.98 & 8.09 &  & 6.94 & 7.20 & 8.53 & 8.69 & 9.64 &  & 5.99 & 6.08 & 7.16 & 10.60 & 8.51 &  & 5.78 & 6.11 & 9.40 & 11.36 & 9.89 \\
UCoFiA &  & 5.07 & 5.75 & 7.26 & 7.59 & 8.13 &  & 7.66 & 7.96 & 8.98 & 8.87 & 10.10 &  & 5.69 & 6.21 & 7.16 & 10.31 & 8.43 &  & 5.00 & 6.33 & 8.82 & 11.26 & 9.81 \\ \hline
\end{tabular}}
\end{table}

==> table-q2-fine-coarse-correlation.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}

%\begin{table}[]
%\caption{\textbf{Coarse \& Fine-grained evaluation}. %\textbf{Metric: Mean R@\{1,5,10\} \textit{ Mean PosRank ($\downarrow$})}
%}
%\label{tab:_q3}
%\centering
%\begin{tabular}{clccccc}
%\hline
%\multirow{2}{*}{Dataset} & \multirow{2}{*}{Method} & \multicolumn{3}{c}{R@\{1,5,10\} ($\uparrow $)} & \multicolumn{2}{c}{PoSRank ($\downarrow$)} \\ 
%\cmidrule{3-5} \cmidrule{6-7}
% &  & \multicolumn{1}{c}{T2V} & \multicolumn{1}{c}{V2T} & Rank & Value & Rank\\ \hline
%\multirow{4}{*}{MSR-VTT} & Frozen & 153.5 & 157.3 & 4& 8.13 & 4\\
% & UCoFiA & 199.2 & 198.5 & 1 & 6.76  & 2\\
% & TS2-Net & \textbf{202.3} & 200.0 & 3 & 6.86 & 3 \\
% & X-CLIP & 200.9 & \textbf{200.1} & 2 & \textbf{6.07} & 1\\
% \hline
%\multirow{4}{*}{VATEX} & Frozen & 207.6 & 208.0 & 4 & 8.55 & 3\\
% & UCoFiA & 243.7 & 267.7 & 3 &8.71 & 4\\
% & TS2-Net & \textbf{247.7} & \textbf{273.1} & 1 & \textbf{8.05} & 1\\
% & X-CLIP & 247.0 & 273.2 & 2 & 8.20 & 2 \\
% \hline
%\multicolumn{1}{l}{\multirow{4}{*}{VLN-UVO}} & Frozen & 115.9 & 116.3 & 4 & 8.17 & 4\\
%\multicolumn{1}{l}{} & UCoFiA & 119.2 & 163.1 & 2 & \textbf{7.56} & 1\\
%\multicolumn{1}{l}{} & TS2-Net & 117.7 & 162.3 & 3 &7.58 & 2 \\
%\multicolumn{1}{l}{} & X-CLIP & \textbf{123.1} & \textbf{170.2} & 1 & 7.67 & 3\\
% \hline
%\multicolumn{1}{l}{\multirow{4}{*}{VLN-OOPS}} & Frozen & 154.4 & 155.8 & 4 & 8.44 & 3 \\
%\multicolumn{1}{l}{} & UCoFiA & 151.8 & 198.7 & 3 & \textbf{8.24} & 1\\
%\multicolumn{1}{l}{} & TS2-Net & 155.5 & 203.6 & 2 & 8.37 & 2\\
%\multicolumn{1}{l}{} & X-CLIP & \textbf{156.8} & \textbf{210.3} & 1 & 8.51 & 4\\
% \hline
%\end{tabular}
%\end{table}




% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \begin{table}[]
% \caption{}
% \centering
% \label{tab:tab:_q3}
% \begin{tabular}{cllrrr}
% \toprule

% \multirow{2}{*}{Dataset} & \multirow{2}{*}{Method} & \multirow{2}{*}{}& \multicolumn{2}{c}{MeanR} & \multicolumn{1}{c}{\multirow{2}{*}{PoSRank}} \\
% \cline{4-5}
%  & & & \multicolumn{1}{c}{T2V} & \multicolumn{1}{c}{V2T} & \multicolumn{1}{c}{} \\ \hline
% \multirow{4}{*}{MSR-VTT} & Frozen & & 28.1 & 24.6 & 8.13 \\
%  & UCoFiA & & 13.7 & 9.8 & 6.76 \\
%  & TS2-Net & & 11.5 & 9.5 & 6.86 \\
%  & X-CLIP & & 12.1 & 10.8 & \textbf{6.07} \\
%  \hline
% \multirow{4}{*}{VATEX} & Frozen & & 7.5 & 7.7 & 8.55 \\
% & UCoFiA & & 3.8 & 2.0 & 8.71 \\ 
%  & TS2-Net & & 3.2 & 1.6 & \textbf{8.05} \\
%  & X-CLIP & & 3.6 & 1.6 & 8.20 \\\hline
% \multicolumn{1}{l}{\multirow{4}{*}{VLN-UVO}} & Frozen & & 57.7 & 50.5 & 8.17 \\
% \multicolumn{1}{l}{} & UCoFiA & & 100.3 & 21.7 & \textbf{7.56}\\
% \multicolumn{1}{l}{} & TS2-Net & & 90.6 & 21.6 & 7.58 \\
% \multicolumn{1}{l}{} & X-CLIP & & 91.3 & 19.4 & 7.67 \\
%  \hline 
% \multicolumn{1}{l}{\multirow{4}{*}{VLN-OOPS}} & Frozen & & 52.1 & 44.6 & 8.44 \\
% \multicolumn{1}{l}{} & UCoFiA & & 57.9 & 14.0 & \textbf{8.24} \\
% \multicolumn{1}{l}{} & TS2-Net & & 56.2 & 14.7 & 8.37 \\
% \multicolumn{1}{l}{} & X-CLIP & & 49.5 & 11.2 & 8.51 \\
% \bottomrule
% \end{tabular}
% \end{table}




%\begin{table}[]
%\caption{\textbf{Correlation Between Coarse \& Fine-Grained Performance}. There is a weak correlation between models' performance coarse and fine-grained metrics, however good coarse-grained performance does not indicate good fine-grained performance.%\textbf{Metric: Mean R@\{1,5,10\} \textit{ Mean PosRank ($\downarrow$})}
%}
%\label{tab:_q2}
%\centering
%\begin{tabular}{clcccccc}
%\toprule
%\multirow{2}{*}{Dataset} & \multirow{2}{*}{Method} & \multicolumn{3}{c}{R@\{1,5,10\} ($\uparrow $)} & & \multicolumn{2}{c}{PoSRank ($\downarrow$)} \\ 
%\cmidrule{3-5} \cmidrule{7-8}
% &  & \multicolumn{1}{c}{T2V} & \multicolumn{1}{c}{V2T} & Rank & & Value & Rank\\ \hline
%\multirow{4}{*}{MSR-VTT} & Frozen & 51.2 & 52.4 & 4& & 8.13 & 4\\
% & X-CLIP & 67.0 & \textbf{66.7} & 2 & & 6.94 & 2\\
%& UCoFiA  & 66.4 & 66.2 & 1 & & \textbf{6.76}  & 3\\
% & TS2-Net & \textbf{67.4} & 66.7  & 3 & & 6.86 & 1 \\

% \midrule
%\multirow{4}{*}{VATEX} & Frozen  & 69.2 & 69.3 & 4 & & 8.55 & 3\\
% & X-CLIP & 82.3 & 91.1 & 2 & & 8.20 & 2 \\
%& UCoFiA  & 81.2 & 89.2 & 3 & &8.71 & 4\\
% & TS2-Net & \textbf{82.6} & \textbf{91.0} & 1 & & \textbf{8.05} & 1\\

%  \midrule
%\multicolumn{1}{l}{\multirow{4}{*}{VLN-UVO}} & Frozen  & 38.6 & 38.8  & 4 & & 8.17 & 4\\
%\multicolumn{1}{l}{} & X-CLIP & \textbf{41.0} & \textbf{56.7} & 1 & & 7.67 & 3\\
%\multicolumn{1}{l}{} & UCoFiA & 39.7 & 54.4 & 2 & & \textbf{7.56} & 1\\ 
%\multicolumn{1}{l}{} & TS2-Net & 39.2 & 54.1 & 3 & &7.58 & 2 \\

%\midrule
%\multicolumn{1}{l}{\multirow{4}{*}{VLN-OOPS}} & Frozen  & 51.5 & 51.9 & 4 &&  8.44 & 3 \\
%\multicolumn{1}{l}{} & X-CLIP & \textbf{52.3} & \textbf{70.1} & 1 & & 8.51 & 4\\
%\multicolumn{1}{l}{} & UCoFiA & 50.6 & 66.2 & 3 & & \textbf{8.24} & 1\\
%\multicolumn{1}{l}{} & TS2-Net & 51.8 & 67.9  & 2 & & 8.37 & 2\\

% \bottomrule
%\end{tabular}
%\end{table}
